Sequential no-Substitution k-Median-Clustering

We study the sample-based k-median clustering objective under a sequential setting without substitutions. In this setting, an i.i.d. sequence of examples is observed. An example can be selected as a center only immediately after it is observed, and it cannot be substituted later. The goal is to select a set of centers with a good k-median cost on the distribution which generated the sequence. We provide an efficient algorithm for this setting, and show that its multiplicative approximation factor is twice the approximation factor of an efficient offline algorithm. In addition, we show that if efficiency requirements are removed, there is an algorithm that can obtain the same approximation factor as the best offline algorithm. We demonstrate in experiments the performance of the efficient algorithm on real data sets. Our code is available at https://github.com/tomhess/No_Substitution_K_Median.

==> section_lowerboundSKM.tex <==

\todosivan{temporary commands}
\newcommand{\cont}{\mathrm{cont}}
\newcommand{\disc}{\mathrm{disc}}
\newcommand{\OPTD}{\OPT_{\disc}}
\newcommand{\OPTC}{\OPT_{\cont}}
\newcommand{\Cost}{\mathrm{cost}}

\section{Lower bounds } \label{section:lowerbounds}
In this section,  we show and discuss extensively  two lower bounds. The lower bound in \thmref{1example} shows that the  factor of $2$  between the clustering found in step 1 and the output of our algorithm  cannot be avoided when $m \rightarrow \infty$. 
The lower bound in  \thmref{2example} shows that the multiplicative factor in \thmref{mtheorem} is tight. Lastly, we discuss an interesting  simple modification to our algorithm, which appears promising at first glance. We believe  that it still obtains  a similar lower bound, which we will show in future work.

In the following lower bounds,  we assume that $\mathcal{A}$ is a $1$-approximation algorithm  for the discrete problem. Such an algorithm always exists, although it might not be efficient. By \eqref{knownlemma}, it is a  $2$-approximation algorithm for the continuous case, i.e, $\beta=2$.  

%have overlooked the computational hardness of the $k$-median objective, in order to focus on the effects of our model's constraints on the guarantees

 
The following theorem shows a lower bound for the ratio between the  risk of $T_{\out}$ and the risk of the clustering found in step 1. It shows that in the worst case, the ratio converges to $2$ when $m$ goes to infinity. 



\begin{theorem}
 \label{thm:1example}Let $\mathcal{A}$ be a $1$-approximation algorithm for the discrete objective. For  any $m \gg k$ and $m_1$ such that $m > m_1 \gg k$, there exists a metric space $(\cX,\rho)$ and a probability distribution $P$ over $\cX$, such that with a constant probability, for any possible setting of $q$ in \algname,  $ R(P,T_{\out})= 2R(P,\mathcal{A}(S_1))-\frac{1}{m_1}$. 
\end{theorem}

\begin{proof} 

Set the distance metric to be the  shortest path in a graph. Set $k=1$. Define an undirected star graph $G=(\cX,E)$ as follows: $\cX=\{o,u_1,\ldots,u_{m_1-1} \}$ and $E=\{\{o,u_i\} \mid i \in [m_1-1]  \}$. Notice that  $\forall i \in [m_1-1], \rho(o,u_i)=1$ and $\forall i\neq j$ such that $i,j\in [m_1-1],\, \rho(u_i,u_j)=2$. Let $P$ be the discrete uniform distribution over $\cX$.  Let us consider the following events:
\begin{enumerate}


\item   $E_1:= \{ o \text{ appears once  in }S_1.\}$ This event occurs with a constant probability,  since 
\[
\P[E_1] = (1-\frac{1}{m_1})^{m_1-1} > \frac{1}{e}.
\]

\item $E_2:= \left\lbrace  \forall T \in S_1^k, |R(P,T)-R(S_1,T)| \leq \sqrt{\frac{k\ln(m_1)+\ln(2e)}{2(m_1-k)}}.\right\rbrace$

By \thmref{BDtheorem},
this event occurs with   probability $1-\frac{1}{2e}$. 
 


\end{enumerate}  
Denote by $E$ the event that both $E_1$ and $E_2$ occur. Notice that $E$  occurs with a constant probability. We now show that if $E$ occurs, then this theorem's claim holds. Assume that $E$ occurs.  $P$ is uniform on $m_1$ elements. Therefore,  $R(P,\{o\})=1-\frac{1}{m_1}$ and $R(P,\{u_i\})=2-\frac{3}{m_1}$.  By $E_1$, $o$ appears in $S_1$, and by $E_2$, for $m_1 \gg k$ then the clustering $\{o\}$ has the best empirical risk on $S_1$. Therefore, $\OPT^{S_1}_{disc}=\{o\}$. Hence, $\mathcal{A}(S_1)=\{o\}$.  By $E_1$,  $o$ appears once in $S_1$, hence for any $q\in (0,1)$, $\qpoint_{S_1}(o,q)=u_i$ for some arbitrary $i$. Therefore, $\qball_{S_1}(o,q)=\cX $ and \algname~selects the first element that it observes in step 2. With a probability of $\frac{m_1-1}{m_1}\geq \frac{1}{2}$,  this  element is some $u_i$,  thus $T_{\out}=\{u_i\}$. Since $R(P,\OPT)=R(P,\{o\})=1-\frac{1}{m_1}$, and $ R(P,T_{\out})=R(P,\{u_i\})=2-\frac{3}{m_1}$, it follows that with a constant probability  $R(P,T_{\out})= 2R(P,\mathcal{A}(S_1))-\frac{1}{m_1}$. 
\end{proof}

In the  theorem above, we showed that the  factor of $2$  between the risks of the clustering found in step 1 and the risk of $T_{\out}$ cannot be avoided for \algname, even with a different setting of $q$. Note that  the  example in the proof of the theorem above can be easily generalized to  $k>1$.\\


The result above, combined with  the guarantee of \eqref{knownlemma}, suggests that   the best multiplicative factor we can hope for \algname, might be $4$.  Indeed, the best multiplicative factor which is possible to obtain by \thmref{mtheorem} is 4, when using a $2$-approximation algorithm for the continuous case. In the lemma below, we show that  for every any $m_1$ and for many choices of $q$ (we discuss later other choices of $q$), the factor of $4$   in \thmref{mtheorem} cannot be improved.


%  However, is the factor of $4$  in the multiplicative error  from \thmref{mtheorem} tight?  from \thmref{2approxBD}, it  follows that the offline algorithm obtains a $2$-approximation, then by \thmref{1example} and our analysis we except that our algorithm truly  obtains ,in the worst case, $4$-approximation. Can we find an example  that indeed obtains this factor?. The following lemma shows that the constant of $4$ in the multiplicative error from \thmref{mtheorem} is tight. 

\begin{theorem} 
\label{thm:2example}Define $\epsilon=\sqrt{\frac{k \ln m_1 +\ln (16)}{2(m_1-k)}}  $. Let $\mathcal{A}$ be a $1$-approximation algorithm for the discrete objective.  For $q=q(m_1)$  such that $q(m_1) \rightarrow 0$ when $m_1 \rightarrow \infty$, and $q(m_1)> 2\epsilon$ for all $m_1$, there exists a metric space $(\cX,\rho)$ and a probability distribution $P$ over $\cX$, such that $\forall \epsilon', \exists M \, s.t. \, \forall m_1\geq M$ with a constant probability,   $\frac{R(P,T_{\out})}{R(P,\OPT)}>4-\epsilon'$. 
\end{theorem}

\begin{proof} 
Set the distance metric to be the  shortest-path in a graph.  Set $k=1$. Define  an undirected graph $G=(\cX,E)$ as follows (see figure \ref{fig:example2fnew}):  $U:=\{u_1,\ldots,u_{m_1} \}$, $Y:=\{y_1, \ldots y_{m_1}\}$, and $\cX:=U \cup Y \cup \{o,v\}$. Define $E_1:=\{\{u,o\} \mid u \in U \}$, $E_2:= \{\{v,y\} \mid y \in Y \}$ and $E_3:=\{ \{o,v\}\}$. Define  $E:=E_1 \cup E_2 \cup E_3$. 

 Define the weight function $W$ over the edges, as follows: \[
\forall e \in E,   W(e) = \begin{cases} 
      1 & e \in E_1\cup E_3, \\
      2-\eta & e \in E_2. \\%      2-\eta & e \in E_3.
   \end{cases}
\]
Where $\eta:=\frac{1}{4m_1}$. 

 
Define the distribution  $P$  as follows:
\[
P(x) = \begin{cases} 
      0 & x=o, \\
      2q /m_1 & x \in Y, \\
      1 / m_1 & x=v,\\
      (1-(2q+\frac{1}{m_1})) / m_1 &  x \in U.
   \end{cases}
\]
If $q<\frac{1-\frac{1}{m_1}}{2}$, then   $P$ is well defined. By the assumptions on $q$, this holds for large enough $m_1$. 
\begin{figure}[H]
   \centering
   \includegraphics[height=1.3in]{example2fignew}
   \caption{The graph defined in \thmref{2example} } 
   \label{fig:example2fnew}
\end{figure}  
 
 
 
 

Let us consider the following events:
\begin{enumerate}
\item   $E_1:=\{o \text{ does not appear   in }S_1\}$. This event occurs with  probability $1$. 

\item   $E_2:=\{v\text{ appears once in }S_1\}.$ This event occurs with  probability  $>\frac{1}{4}$, since
\[
\P[E_2] = (1-\frac{1}{m_1})^{m_1-1} > \frac{1}{e}>\frac{1}{4}.
\]

\item $E_3:=\{\text{Number of instances of vertices from } Y \text{ in }S_1 \text{ is larger than }q m_1\}$. The expected  number of instances from $Y$ in $S_1$ is $2q|S_1|$. Hence, by Hoeffding's inequality,  this event occurs with  probability $1-e^{-2m_1q^2}$. By the assumption  $q>2\epsilon$, we get that this event occurs with probability $>1-\frac{1}{8}$.


\item  $E_4:= \{\forall T\in S_1^k \, |R(P,T)-R(S_1,T)| \leq \epsilon    \}$. By \thmref{BDtheorem}, this event occurs with  probability $\geq 1-\frac{1}{16}$. 
\end{enumerate}  

Denote by $E$ the event that all of the  above events occur.  Notice that $E$ occurs with a  probability larger  than $\frac{1}{16}$. We now show that if $E$ occurs then this theorem's claim holds. Assume that $E$ occurs.   We have \[R(P,\{o\})=\left( 1-(2q+\frac{1}{m_1})\right)+\frac{1}{m_1}+(3-\eta)2q<1-2q+3 \cdot 2 q=  1+4q.\]
For any $u\in U$, 
\begin{align*}
 R(P,\{u\})&= 
 2(1-(2q+\frac{1}{m_1})(1-\frac{1}{m_1})+\frac{2}{m_1} +(4-\eta)2q\\
  &=2+4q-2\frac{1-(2q+\frac{1}{m_1})}{m_1} -2q \eta>2+4q-\frac{2}{m_1}-q > 2+q.
\end{align*} The second to last inequality follows from the definition of $\eta$. The last inequality follows from  the assumption $q>2\epsilon>2\sqrt{\frac{\ln(16)}{m_1}}$.

Also, 
\[R(P,\{v\})= 2\left(1-(2q+\frac{1}{m_1})\right)  +(2-\eta)2q=2-\frac{2}{m_1}-2q\eta<2,
\] 

and for any $y\in Y$, 
\begin{align*}
 R(P,\{y\})&=(4-\eta)\left(1-(2q+\frac{1}{m_1})\right)+(2-\eta)\frac{1}{m_1}+(4-\eta)2q(1-\frac{1}{m_1})\\
 &=4-\frac{2+8q}{m_1}-\eta(1-\frac{2q}{m_1})>4-(\frac{3}{m_1}+\eta)>4-\frac{4}{m_1}
.
\end{align*}
The first inequality holds for a large enough $m_1$. The second inequality follows from the definition of $\eta$. 



By $E_1$, $o$ does not appear in $S_1$, and by $E_2$, $v$ appears at least once in $S_1$. Therefore, $v$ has a better risk on the distribution than the rest of the points in $S_1$.


Also, by $E_4$ and the assumption $q>2\epsilon$, $v$  has the best empirical risk on $S_1$. Therefore,  $\OPTD^{S_1}=\{v\}$. Hence, $\mathcal{A}(S_1)=\{v\}$.   By $E_2$, $v$ appears once in $S_1$. By $E_3$, the number of instances of vertices from $Y$ is at least $qm_1$. Since the points in $Y$ are the closest to $v$,  we have $\qpoint_{S_1}(v,q)=y'$ for some arbitrary $y' \in Y$. Therefore, $ \qball_{S_1}(v,q)=\{ v\} \cup Y$ and \algname~selects the first element that it observes in step 2 from $\{ v\} \cup Y$. With a probability $\frac{2q}{2q+\frac{1}{m_1}}>\frac{2}{3}$,  the first element that  \algname~observes is some $y''\in Y$, and thus with a constant probability $T_{\out}=\{y''\}$. 

Notice that for any $q$ which satisfies the condition of the theorem for a large enough $m_1$,  $\OPT=\{o\}$. Therefore, with a constant probability, the ratio between  $R(P,T_{\out})$ and $R(P,\OPT)$ is $> \frac{4-\frac{4}{m_1}}{1+4q}$. Recall that $q(m_1)\longrightarrow 0$ when $m_1 \rightarrow \infty$. Therefore, this ratio tends to $4$ as $m_1$ grows. This completes the proof. 
%The distance metric is the  shortest path in a weighted a graph. Let $k=2$. Define graph $G=(\cX,E)$, see figure \ref{fig:example2f},  such that  $O=\{o_1,o_2 \}$, $U=U_1 \cup U_2$ such that $U_i=\{u^i_1, \ldots u^i_{m_1}\}$, $D=\{d_1,d_2\}$, and $V=\{v_1,v_2\}$ Define the vertices $\cX=O \cup U \cup D \cup V$. Define $E_1=\{(u,o_1) \mid u \in U \}$, $E_2= \{(u^i_j,d_i) \mid i \in [1,2], j \in [1,m_1]\}$ and $E_3=\{ (d_1,v_1),(d_2,v_2)\}$. Define the edges $E=E_1 \cup E_2 \cup E_3$. 
%
% Define the weight function $W$ over the edges, as follows: \[
%\forall e \in E,   W(e) = \begin{cases} 
%      1 & e \in E_1, \\
%      2 & e \in E_2, \\
%      2-\frac{1}{2^{m_1}} & e \in E_3.
%   \end{cases}
%\]
% Define $\epsilon=\sqrt{\frac{k\ln m_1 +\ln (\frac{1}{\delta})}{m_1-k}}$, This is exactly the accuracy of the empirical risk by \thmref{BDtheorem} for sample $S_1$.
%Define the distribution  $P$  as follows:
%\[
%P(x) = \begin{cases} 
%      \frac{1}{2^{m_1}} & x \in O, \\
%      \frac{4}{m_1} & x \in D, \\
%      2 \epsilon & x \in V, \\
%      \frac{1-2(2\epsilon+\frac{4}{m_1}+ \frac{1}{2^{m_1}})}{2m_1} &  x \in U.
%   \end{cases}
%\]
% $P$ sums to $1$,  for large enough $m_1$.
%\begin{figure}[H]
%   \centering
%   \includegraphics[height=3in]{example2fig}
%   \caption{Example LaTeX Figure} 
%   \label{fig:example2f}
%\end{figure} 
%  Let us define the following events:
%\begin{enumerate}
%\item  The difference between the empirical risk on $S_1$ and the true risk of every point in $S_1$ is $\epsilon$. This event occurs with  probability $1-\delta$ by \thmref{BDtheorem} 
%
%\item   $d_1$ and $d_2$ appear at least 1 time in $S_1$. This event occurs with constant probability  since 
%\[
%\P[d_1 \notin S_1] = (1-\frac{4}{m_1})^{m_1} > e^{-4}
%\]
%Hence, by union bound 
%\[
%\P[D \subseteq S_1]>1-2e^{-4}
%\]
%\item $o_1$ and $o_2$ do not appear in $S_1$. This event occurs with very big constant probability since  their probability mass are negligence.
%\item $v_1$ and $v_2$ appear more than $q$ times in the data. This event occurs with constant probability, since the expectation of appearance in $S_1$ of $v_i$ is $2q$.
%\end{enumerate} 
%Denote by $E$, the event that the latter events occur simultaneously. Notice that  for large enough $m$, $E$  occurs with constant probability. In the following, we show that if $E$ occurs, then the theorem term holds . Assume $E$ occurs. Notice that $R(P,O)=1+O(\frac{1}{\sqrt{m_1}})$, $R(P,D)=2-O(\frac{1}{2^m})$, $R(P,V)=4-O(\frac{1}{\sqrt{m_1}})$ and $R(P,\{u_i^1,u_j^2\})=2+2\epsilon-\frac{1}{2^m}$. Therefore,   $\OPT^{S_1}_{disc}=D$. Since, every $o\in O$ does not appear in $S_1$ by event 3, $d_1$ and $d_2$ appear in $S_1$ by event 2 and $D$ has the best empirical risk on $S_1$ by event 1. Hence, $\mathcal{A}(S_1)=D$. $v_i$ is the closet point to $d_i$ in $S_1$. In addition, by event 4, $v_1$ and $v_2$ appear more than $q$ times in $S_1$ and hence, $d_i^q=v_i$ for $i \in \{1,2\}$. Therefore, algorithm \ref{SKM} selects the first element it observes from the balls $\ball(d_i,v_i)=\{d_i,v_i,o_2\}$.  Notice that the probability mass of $v_i$ is much larger than the probability mass of $d_i$ and $o_2$. Hence, with constant probability,  the first element observed in step 2, which contained in $\ball(d_i,v_i)$, is $v_i$. Thus, $T_{\out}=V$. Therefore, the ratio between the $T_{\out}$ and $\OPT$ is $\frac{4-\frac{1}{m_1}}{1+\frac{1}{\sqrt{m_1}}}$. This completes the proof.
\end{proof}


In the  theorem above we show that our analysis for the multiplicative error is tight. In addition, notice that the above construction can be easily generalized to  $k>2$. However, this theorem does not show guarantees for all possible choices of $q$. We now consider the case where $q$ is some constant and show that choosing a constant $q$  is not beneficial. If $q$ is a constant, then the additive error does not converge to zero. For example, consider the case where $k=2$ and $R(P,\OPT)=0$. The probability mass of one of the clusters is $\frac{q}{2}$ and the distance between the two clusters  is 1. Denote the center of the small cluster by $c$.  With a constant probability, the algorithm selects a point which is outside the small cluster, since half of the probability mass of  $\qball_{S_1}(c,q)$ is of points outside the small cluster. Hence,with a constant probability the algorithm selects  $T_{\out}$ such that $R(P,T_{\out})=\frac{q}{2}$. Hence, the additive error is $\frac{q}{2}$, which is a constant and does not converges to $0$ when $m \longrightarrow \infty$. Note that this example holds for any $q$, not just a constant. Hence, it disqualifies any $q$ that is larger than the allowed additive error.   The other case that the theorem above does not handle is $q \leq \epsilon$. We intend to analyze  this case in  future work.
%Basically it happens since either  the ratio between $m_1$ and $m_2$ sis constant and then $B$ and $\hat{B}$ can be very far, and hence with constant probability we might wait all step 2 without picking any point. Otherwise $m_2>>m_1$ might work but our understanding of the underlyign distribution is much worse and hence the additive error guarntee would be much worse with respect to $m$.



Can changing the method of selection in step 2  improve the multiplicative factor? 
 Consider a different way to select centers in step 2 in \algname. Suppose centers are selected by the cost that they induce  on the cluster, and not by their closeness to the  centers of the clustering $\mathcal{A}(S_1)$. In order to define the modified algorithm, we need to slightly change the notation.
Consider a set $S=(x_1,\ldots,x_n)$. For $x_i \in S_1$ and $C \subseteq S_1$, define $t_{x_i,C}(s): \cX  \rightarrow \{ 0, 1 \}$ s.t.  $t_{C,x_i}(x)=\mathbb{I}[\Cost(C,x)\leq \Cost(C,x_i) ]$.  \todosivan{clashes with definition of $\hat{B}$?} Define $B_{C,x_i}(s)=\P_{s \sim P}[\Cost(C,s) \leq \Cost(C,x_i) ]$ and $\hat{B}_{C,x_i}= \frac{1}{|S_1|-1}\sum_{l \in [n]: l \neq i}t_{C,x_i}(s)$. 
Let  $q \in [0,1]$. Define a quantile point of a cluster by $a^{C,q}:= \argmin_{\{y \in S_1 \mid \hat{B}_{C,y} \geq q\}} \hat{B}_{C,y} $. Recall that the original definition of quantile was  relative to a single point, the cluster center, while in this definition it is relative to the entire set of points in the cluster. Define a risk-closed ball $\ball_R(C,x_i)=\{  x \in \cX \mid \Cost(C,x) \leq \Cost(C,x_i) \}$. The only modifications in \algname~are as follows: in line 7  compute $a^{C_i,q}$ instead of $c_i^q$. In line 9,  change $\ball(c_i,r^q_{c_i})$ to $\ball_R(C_i,a^{C_i,q})$.   

 

If the modified \algname~selects $t_i$ for each cluster in line 8, then this suggested decision rule  clearly obtains a better empirical risk on $S_1$ compared to the decision rule used in \algname, since $\ball_R(C_i,a^{C_i,q})\subseteq  \ball(c_i,r^q_{c_i})$. However,  proving an analog theorem of \thmref{mtheorem} for this modification  is not trivial, since the sample compression technique used in \lemref{approxballslemma} cannot be used easily in this case.  Notice that the  example of  \thmref{2example} cannot be used to construct a lower bound for the proposed modification. Nonetheless, we believe that  even for the modified version, the worst case remains almost the same. This will be shown in future work. 

%\begin{theorem}
%\label{thm:3example}  Let $\mathcal{A}$ be a $1-$approximation algorithm for the discrete case. Fix $k\geq 4$. For the modified version of \algname~suggested above with $ \frac{1}{8k^2} \geq q\geq \frac{2k}{m_1}$, 
% there exist a metric space $(\cX,\rho)$ and a probability distribution $\cP$ over $\cX$, such that $\forall \epsilon' \, \exists M \,s.t. \, \forall m_1 \geq M$ with constant probability,   $\frac{R(P,T_{\out})}{R(P,\OPT})>4-\frac{8}{k}-\epsilon'$. 
%
%\end{theorem} 
%\begin{proof}
%Set the distance metric to be the  shortest path in a graph.
%Define an undirected graph $G=(\cX,E)$ (see figure \ref{fig:example3fnew})  as follows: $T^j= \{ t_i^j \mid i \in [k] \}, T=\bigcup_{j \in [k]}T^j, O = \{ o_1, \ldots o_k \}
%,D= \{ d_1,\ldots d_k \}$, and $\cX=T \cup O \cup D$.
% Define $ E_1=\{\{o_i,t^j_i\} \mid i,j \in [k]\}$, \\ $E_2=\{\{d_i,t_j^i\} \mid i,j \in [k]  \}$ ,  and $E=E_1 \cup E_2$. Define the weight function $W$ over the edges, as follows:
% \[W(e) = \begin{cases} 
%      1 & e \in E_1, \\
%      2-4/k & e \in E_2 \text{ and } e=(d_i,t_1^i), \\
%      2-2/k &  else. 
%   \end{cases}
%\] 
%
%
%Define the distribution  $P$ as follows:
%\[
%P(x) = \begin{cases} 
%      0 & x \in O, \\
%      k/m_1 & x \in D, \\
%      2q & x=t^j_1 \text{ and } j\in [k], \\
%      (1-k(\frac{k}{m_1}+2q)) /(k^2-k) &  \text{else.}
%   \end{cases}
%\]
%For $q<\frac{1}{2}(\frac{1}{k}-\frac{k}{m_1})$, $P$ is well defined. By the assumption on $q$, this holds for large enough $m_1$.
%\begin{figure}[H]
%   \centering
%   \includegraphics[height=2.6in]{example3fig}
%   \caption{The graph defined in \thmref{3example} } 
%   \label{fig:example3fnew}
%\end{figure} 
%
% Let us consider the following events:
%\begin{enumerate}
%
%
%\item   $E_1:=\{\text{Every }d\in D\text{ appears at least once in }S_1\text{ and at most }2k-1.\}$ The expected number  of instances of each $d \in D$ in $S_1$ is $k$. Hence, by Bernstein's inequality, the event that $d\in D$ appears at least once and at most $2k-1$, occurs with probability larger than  
%$1-2e^{-k}$.
% Hence, by applying the union bound, the above event occurs, for every $d\in D$ simultaneously, with probability 
%$
%\geq 1-2ke^{-k}>1-3/10
%$.
%
%\item $E_2:=\{ \text{Every }o\in O\text{ does not appear in }S_1\}.$ This event occurs with  probability $1$.
%
%\item $E_3:=\{\text{Every }v_1^j\text{ for }j\in [k]\text{  appears more than }q |S_1|\text{ times in the data}.\}$ The expected number of instances of each $v_1^j$ in $S_1$ is $2q|S_1|$. Hence, by Bernstein's inequality, the event that some $v_1^j$ appears at least $q|S_1|$ occurs with probability larger than $1-2e^{m_1q}$. Hence, by applying the union bound, the above event occurs, for every $v_1^j$, with probability $1-2ke^{-m_1q}$. Recall that $q\geq \frac{1}{m_1}$. Therefore,  probability is larger than $1-2ke^{-k}>1-3/10$.
%
%\item $E_4:=\{\text{Every element in }\{ t \in T \mid \forall j \in [k], t \neq t_1^j \}\text{ appears at most }\frac{2}{k^2}|S_1|\}.$ The expected  number of instances of each such $t$ in $S_1$ is at most $\frac{1}{k^2} |S_1|$. Hence, by Hoeffding's inequality, the event that $t \in \{t \in T \mid \forall j \in [k], t \neq t_1^j \} $ 
%appears at most $\frac{2}{k^2}|S_1|$ occurs with probability larger than $1-2e^{\frac{1}{k^2}m_1}$. Hence, by applying the union bound, the above event occurs, for every $t \in \{t \in T \mid \forall j \in [k], t \neq t_1^j \} $ simultaneously, with probability $\geq 1-2k^2e^{-\frac{1}{k^2}m_1}$. For large enough $m_1$, this probability is larger than $1-1/20$.
%
%\item $E_5:\{$ Number of instances of any $T^j$ is at least $(k-\frac{1}{k^2})|S_1| \}$.  The expected  number of instances of each such $T^j$ in $S_1$ is $k|S_1|$. Hence, by Hoeffding's inequality, the event that the number of instances of $T^j$
%is  at least  $(k-\frac{1}{k^2})$ occurs with probability larger than $1-2e^{\frac{1}{k^4}m_1}$. Hence, by applying the union bound, the above event occurs, for any $T^j$  simultaneously, with probability $\geq 1-2ke^{\frac{1}{k^4}m_1}$. For large enough $m_1$, this probability is larger than $1-1/20$.
%
%
%
%
%\item  $E_6:= \left\lbrace\forall T\in S_1^k, |R(P,T)-R(S_1,T)| \leq \sqrt{\frac{k\ln(m_1)+\ln(5)}{m_1-k}}:=\epsilon \right\rbrace$. By \thmref{BDtheorem}, this event occurs with  probability $ \geq 1-1/5$.  
%\end{enumerate} 
%
%Denote by $E$, the event that all of the above events occur. Notice that $E$ occurs with  probability $>1/10$. We now show that if $E$ occurs, then this theorem's claim  holds . Assume $E$ occurs. we have  \begin{align*}
%R(P,O)=1(1-\frac{k^2}{m_1})+(3-\frac{4}{k})(\frac{k^2}{m_1})< 1+2\frac{k^2}{m_1},
%\end{align*}
%
%\begin{align*}
%R(P,D)=2qk(2-\frac{4}{k}+(1-2qk)(2-\frac{2}{k})=2-4q-\frac{2}{k}\leq 2-\frac{2}{k}, 
%\end{align*}
%
%
% For any $j\in [k]$,
%
% \begin{align*}
%  R(P,\{t^j_1,t^j_2,\ldots,t^j_k  \})&=  2(1-k(\frac{k}{m_1}+2q)))+(2-\frac{4}{k})2q+2q(k-1)(2-\frac{2}{k}) \\ 
%  &\geq 2-\frac{2k^2}{m_1}-8q  
%\end{align*}
%For large enough $m_1$ and $q<\frac{1}{8}k^2$, we get 
%\[
% R(P,\{t^j_1,t^j_2,\ldots,t^j_k  \}) > 2-\frac{1}{k}
%\]
%
%\begin{align*}
% R(P,\{t_1^1,t_1^2,\ldots,t_1^k \})=(4-\frac{6}{k})(1-k(\frac{k}{m_1}+2q))+(2-\frac{4}{k})\frac{k^2}{m_1} \geq 4-\frac{6}{k}-8qk-4\frac{k^2}{m_1}.
%\end{align*}
%For large enough $m_1$ and $q<\frac{1}{8}k^2$, we get 
%\[
%R(P,\{t_1^1,t_1^2,\ldots,t_1^k \}) >4-\frac{8}{k}.
%\]
%Notice that all the other   possible clusterings, which their risk was not calculated explicitly,  with centers with probability mass larger than $0$,  have risk close to 4.
%
%  By $E_2$, every $o\in O$ does not appear in $S_1$  and by $E_1$, every $d\in D$ appears at least once in $S_1$. Therefore, $D$ has the best risk  on the distribution than the rest of the clustering induced by points in $S_1$. By  $E_6$, for large enough $m_1$, $D$ has also the best empirical risk on $S_1$. Hence,  $\OPT^{S_1}_{disc}=D$ and  $\mathcal{A}(S_1)=D$. 
%  
%  
%  Denote the clusters determined by $D$  by $D_i= \{d_i,t_1^i,t_2^i,\ldots,t_k^i \}$ ( Notice that each point in $D_i$ could has  more than one instance in $D_i$). 
%  
%Notice that $R(D_i,t_1^i)<2-\frac{6}{k}$. By $E_4$ and $E_5$, the ratio between the number of instances of each $t^i_j$ and the size of $T^i$ is $<\frac{2}{k-1}$. Hence, for large enough $m_1$, $j \neq i$, $R(D_i,t^i_j)>2-\frac{6}{k}$.
%Hence, the element which obtains the second best risk as center for $D_i^{S_1}$ is $t_1^i$.  Moreover, by  $E_3$, any $v_1^i$ for $i\in [k]$ appears more than $q|S_1|$ times in $S_1$ and by $E_1$, every $d_i$ appears at most $2k<q|S_1|$.   Hence, $D_i^q=v_1^i$ for $i \in [k]$.  Therefore,  \algname~selects the first element that it observes from each ball $\ball_R(C_i,a^{D_i,q})=\{d_i,v_1^i\}$.   With probability of  $\frac{2q}{2q+\frac{k}{m_1}} \geq \frac{2q}{2q+\frac{q}{2}}=0.8$ this element is  $v_1^i$.  Thus, with a constant probability  $T_{\out}=\{v_1^1,v_1^2,\ldots,v_1^k \}$. Notice that for large enough $m_1$, $\OPT=O$. Therefore, the ratio between the $R(P,T_{\out})$ and $R(P,\OPT)$ is $\frac{4-\frac{8}{k}}{1+2\frac{k^2}{m_1}}$. This completes the proof.
%
%
%
%
%\end{proof}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "SKM_v1"
%%% End:


==> section_mainresults.tex <==
\section{Main Results}


\todosivani{todo}

%\todosivan{later: mention this in the right way}
%We show  below, in Section \ref{section:lowerbounds}, that this ratio is unavoidable for our algorithm if the algorithm does not know $\cX$ in advance.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

